The Talented Mr. Inversive Triangle in the Elliptic Billiard

Inverting the vertices of elliptic billiard N-periodics with respect to a circle centered on one focus yields a new "focus-inversive" family inscribed in Pascal's Lima\c{c}on. The following are some of its surprising invariants: (i) perimeter, (ii) sum of cosines, and (iii) sum of distances from inversion center (the focus) to vertices. We prove these for the N=3 case, showing that this family (a) has a stationary Gergonne point, (b) is a 3-periodic family of a second, rigidly moving elliptic billiard, and (c) the loci of incenter, barycenter, circumcenter, orthocenter, nine-point center, and a great many other triangle centers are circles.

==> 002_refcheck.tex <==
\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

==> 030_n3_further_invariants.tex <==
As noted in \cref{tab:symbols}, let $d_{1,i}=|P_i-f_1|$.

\begin{proposition}
For $N=3$, the sum of focus-inverse spoke lengths is invariant and given by:

\[  \sum\frac{1}{d_{1,i}}=\frac {{a}^{2}+{b}^{2}+\delta}{a{b}^{
2}}
\]
%= {\frac {J\sqrt{2}\sqrt{ J\,L+\sqrt {9-2\,JL}-3 }}{ J L-4 }}
% =\left(\frac{2J}{JL-4}\right)^2

\end{proposition}

\noindent Referring to \cref{fig:inv-pedals}:

\begin{proposition}
For $N=3$, the area product $A_1^\dagger A_2^\dagger$ of the two focus-inversive triangles is given by:

\[ A_1^\dagger A_2^\dagger= \frac{\rho^8}{8 a^8 b^2}  \left[\left( {a}^{4}+2\,{a}^{2}{b}^{2}+4\,{b}^{4} \right)\delta +  \frac{3 a^{4} b^{2}}{2}+a^6+4\,{b}^{6} \right]
\]
\end{proposition}

\begin{observation}
The areas of both pedal triangles of the focus-inversives with respect to the respective foci are dynamically equal.
\end{observation}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/0130_n3_inv_pedals.eps}
    \caption{$f_1$- and $f_2$-inversive triangles are shown (pink). The product of their areas is invariant. Also shown are the $f_1$- and $f_2$-pedal polygons (orange) to said triangles. Their areas are variable but dynamically equal. \href{https://youtu.be/0L2uMk2xyKk}{Video}}
    \label{fig:inv-pedals}
\end{figure}





==> 220_app_n3.tex <==
Let $P_i=(x_i,y_i)/q_i$, $i=1,2,3$, denote the 3-periodic vertices, given by \cite{garcia2019-incenter}:

\begin{align*}
q_1&=1\\
%\label{eqn:p2}
x_{2}&=-{b}^{4} \left(  \left(   a^2+{b}^{2}\right)k_1 -{a}^{2}  \right) x_1^{3}-2\,{a}^{4}{b}^{2} k_2  x_1^{2}{y_1}\\
&+{a}^{4} \left(  ({a
}^{2}-3\, {b}^{2})k_1+{b}^{2}
 \right) {x_1}\,y_1^{2}-2{a}^{6} k_2 y_1^{3}\\
y_{2}&= 2{b}^{6} k_2 x_1^{3}+{b}^{4}\left(  ({b
 }^{2}-3\, {a}^{2}) k_1  +{a}^{2}
  \right) x_1^{2}{y_1}\\
&+  2\,{a}^{2} {b}^{4}k_2 {x_1} y_1^{2} -{
a}^{4}  \left(  \left(   a^2+{b}^{2}\right)k_1  -{b}^{2}  \right)  y_1^{3}
\\
q_2&={b}^{4} \left( a^2-c^2k_1   \right)
x_1^{2}+{a}^{4} \left(  {b}^{2}+c^2k_1  
 \right) y_1^{2} - 2\, {a}^{2}{b}^{2}{c^2}k_2 {x_1}\,{
y_1} \\
x_{3}&= {b}^{4} \left( {a}^{2}- \left( {b}^{2}+{a}^{2} \right) \right)
 k_1  x_1^{3} +2\,{a}^{4}{b}^{2}k_2  x_1^{2}{ y_1}\\
 &+{a}^{4} \left( 
  k_1 \left( {a}^{2}-3\,{b}^{2}
 \right) +{b}^{2} \right) { x_1}\, y_1^{2} +2\, {a}^{6} k_2 y_1^{3}
\\
y_{3}&= -2\, {b}^{6} k_2 x_1^{3}+{b}^{4} \left( {a}^{2}+ \left( {b}^{2}-3\,{a}^{2} \right)    k_1 \right) {{ x_1}}^{2}{ y_1}
\\
& -2\,{a}^{2}  {b}^{4} k_2  x_1 y_1^{2}+
 {a}^{4} \left( {b}^{2}- \left( {b}^{2}+{a}^{2} \right)   k_1 \right)\,  y_1^{3},
\\
q_3&= {b}^{4} \left( {a}^{2}-{c^2}k_1   \right) x_1^{2}+{a}^{4} \left( {b}^{2}+c^2k_1  \right)  y_1^{2}+2\,{a}^{2}{b}^{
2} c^2 k_2\, { x_1}\,{ y_1}.
\end{align*}

\noindent where:


\begin{align*}
k_1&=\frac{d_1^2\delta_1^2}{\,d_2}=\cos^2{\alpha},\\
k_2&=\frac{ \delta_1d_1^2}{d_2 }\sqrt{ d_2 -d_1^4\delta_1^2}=\sin{\alpha}\cos\alpha\\
c^2&=a^2-b^2,\;\; d_1=(a\,b/c)^2,\;\;d_2={b}^{4}x_1^2 +{a}^{4}y_1^2\\
\delta&=\sqrt{a^4+b^4-a^2 b^2},\;\;\delta_1=\sqrt{2 \delta-a^2-b^2}
\end{align*}

\noindent where $\alpha$, though not used here, is the angle of segment $P_1 P_2$ (and $P_1 P_3$) with respect to the normal at $P_1$.

\noindent The caustic is the ellipse:

\[\frac{x^2}{a''^2}+\frac{y^2}{b''^2}-1=0, \;\; a''=\frac{a( \delta-b^2)}{{a^2-b^2}}, \;\; b''=\frac{b(a^2-\delta)}{{a^2-b^2}}  \]


==> 225_app_x7.tex <==
\textcolor{red}{mark: por favor checar a algebra e confirmar q funciona numericamente?}

The x-coordinate of $X_7^\dagger=(x_7^\dagger,0)$ is given by:

{\small
\begin{align*}
    x_7^\dagger & = k_1/k_2 \\
    k_1 & = a^2 b^4 \left(a^2-a c-b^2-1\right) \left(a^8 \left(3 b^2+2  \delta\right)+4 a^6 b^2  k_3 +a^4 \left(6 b^4  \delta+7 b^6\right)+4 a^2 b^6 \delta+2 a^{10}+8 b^8  k_3 \right)\\
    &+(a-c) k_4 \left(a^2 c \left(2 b^2+1\right)+a^3-k_3(a+c) \right) \left(b^2 k_4 -\left( \delta \left(a c \left(a^2+b^2\right)+k_7\right)+a c k_7+a^6+b^6\right) k_5\right) \\
     k_2 & = a^2 (a-c) \left(-2 b^2 \left( \delta \left(a c (a^2+b^2\right)+k_7\right)+a c k_7+a^6+b^6\right) k_6\\
     &+4 a^2 b^{10}  \delta+a^4 b^8 \left(7 b^2+6  \delta\right)+4 a^6 b^6  k_3 +a^8 b^4 \left(3 b^2+2  \delta\right)+2 a^{10} b^4+8 b^{12}  k_3 )\\
    k_3 & = b^2+\delta\\
    k_4 & =\sqrt{a^8 \left(3 b^2+2  \delta\right)+4 a^6 b^2  k_3 +a^4 \left(6 b^4  \delta+7 b^6\right)+4 a^2 b^6  \delta+2 a^{10}+8 b^8  k_3 } \\
    k_5 & = \sqrt{\frac{\left(a^2+b^2+ \delta\right)^2}{(a-c)^2}+\frac{b^4 \left(-a^2 b^2+a^4+2 b^2  k_3 \right) \left(a^4 \left(b^2+2  \delta\right)+a^2 \left(2 b^2  \delta+b^4\right)+2 a^6+2 b^4  k_3 \right)}{\left( \delta \left(a c \left(a^2+b^2\right)+k_7\right)+a c k_7+a^6+b^6\right)^2}} \\
    k_6 & = k_4 k_5\\
    k_7 & = a^4+b^4
\end{align*}
}

==> _app/120_app_vertices_caustics.tex <==
\subsection{N=3 Vertices \& Caustic}
\label{app:3-periodic}
\input{app/230_app_n3_vtx}

\subsection{N=4 Vertices \& Caustic}
\label{app:4-periodic}
\input{app/240_app_n4_vtx}

\subsection{N=5 Vertices \& Caustic}
\label{app:5-periodic}
\input{app/250_app_n5_vtx}

\subsection{N=6 Vertices \& Caustic}
\label{app:6-periodic}
\input{app/260_app_n6}

\subsection{N=7 Caustic}
\label{app:7-periodic}
\input{app/270_app_n7}

\subsection{N=8 Vertices \& Caustic}
\label{app:8-periodic}
\input{app/280_app_n8}

==> _app/310_app_regular_polys.tex <==
\begin{align*}
    J=&  \frac{\sqrt{2}}{2a}\sqrt{1-\cos(2\pi/N)}
\\
    L=& 2 N a^2 J \\
    k_{101}=& JL-N \\
    k_{102}=&  \cos^N \left[  \frac {\pi\, \left( N-2 \right) }{N}\right]   =\left(\frac{J L}{N}-1\right) ^{N}
\\
    k_{103}=& ...\\
    k_{104}=& ... \\
    k_{105}=& ... \\
    k_{106}=& ... \\
    k_{107}=& ... \\
    k_{108}=& 
\end{align*}

==> _app/320_app_invariant_numeric.tex <==
The tables below present values for $J$, $L$, $J L$, and $k_i,i=1{\ldots}8$, $N=3{\ldots}12$ for a few values of $a/b$, obtained from numerical simulation. Numbers show approximated to 3 decimals.

\subsection{$a/b=1$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.866 & 0.707 & 0.588 & 0.5 & 0.434 & 0.383 & 0.342 & 0.309 & 0.282 & 0.259 \\
 \text{L} & 5.196 & 5.657 & 5.878 & 6 & 6.074 & 6.123 & 6.156 & 6.18 & 6.198 & 6.212 \\
 \text{JL} & 4.5 & 4 & 3.455 & 3 & 2.636 & 2.343 & 2.106 & 1.91 & 1.746 & 1.608 \\
 k_{101} & 1.5 & 0 & -1.545 & -3 & -4.364 & -5.657 & -6.894 & -8.09 & -9.254 & -10.392 \\
 k_{102} & 0.125 & 0 & -0.003 & 0.016 & -0.037 & 0.062 & -0.091 & 0.12 & -0.149 & 0.178 \\
 k_{103} & 4 & \text{n/a} & 1.528 & \text{n/a} & 1.232 & \text{n/a} & 1.132 & \text{n/a} & 1.086 & \text{n/a} \\
 k_{104} & -1.5 & -4 & -4.045 & -3 & -1.558 & 0 & 1.563 & 3.09 & 4.57 & 6\\
 k_{105} & 0.125 & \text{n/a} & 0.347 & \text{n/a} & 0.482 & \text{n/a} & 0.571 & \text{n/a} & 0.635 & \text{n/a} \\
 k_{106} & \text{n/a} & 8 & \text{n/a} & 9 & \text{n/a} & 9.373 & \text{n/a} & 9.549 & \text{n/a} & 9.646 \\
 k_{107} & \text{n/a} & 0.5 & \text{n/a} & \text{n/a} & \text{n/a} & 0.622 & \text{n/a} & \text{n/a} & \text{n/a} & 0.707 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.16 & \text{n/a} & \text{n/a} & \text{n/a} & 1.826 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=1.25$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.752 & 0.625 & 0.522 & 0.444 & 0.386 & 0.341 & 0.305 & 0.275 & 0.251 & 0.231 \\
 \text{L} & 5.916 & 6.403 & 6.644 & 6.778 & 6.86 & 6.913 & 6.95 & 6.977 & 6.996 & 7.011 \\
 \text{JL} & 4.449 & 4 & 3.465 & 3.012 & 2.648 & 2.355 & 2.117 & 1.92 & 1.756 & 1.617 \\
 k_{101} & 1.449 & 0 & -1.535 & -2.988 & -4.352 & -5.645 & -6.883 & -8.08 & -9.244 & -10.383 \\
 k_{102} & 0.112 & 0 & -0.003 & 0.015 & -0.036 & 0.061 & -0.09 & 0.119 & -0.148 & 0.176 \\
 k_{103} & 4.451 & \text{n/a} & 1.546 & \text{n/a} & 1.238 & \text{n/a} & 1.135 & \text{n/a} & 1.088 & \text{n/a} \\
 k_{104} & -1.449 & -4 & -4.035 & -2.988 & -1.551 & 0 & 1.557 & 3.08 & 4.556 & 5.984 \\
 k_{105} & 0.112 & \text{n/a} & 0.342 & \text{n/a} & 0.479 & \text{n/a} & 0.569 & \text{n/a} & 0.633 & \text{n/a} \\
 k_{106} & \text{n/a} & 12.5 & \text{n/a} & 14.043 & \text{n/a} & 14.632 & \text{n/a} & 14.912 & \text{n/a} & 15.066 \\
 k_{107} & \text{n/a} & 0.476 & \text{n/a} & \text{n/a} & \text{n/a} & 0.621 & \text{n/a} & \text{n/a} & \text{n/a} & 0.706 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.211 & \text{n/a} & \text{n/a} & \text{n/a} & 1.836 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=1.5$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
\hline
 \text{J} & 0.648 & 0.555 & 0.467 & 0.4 & 0.348 & 0.308 & 0.275 & 0.249 & 0.227 & 0.209 \\
 \text{L} & 6.738 & 7.211 & 7.459 & 7.6 & 7.687 & 7.743 & 7.783 & 7.811 & 7.832 & 7.848 \\
 \text{JL} & 4.363 & 4 & 3.487 & 3.04 & 2.676 & 2.382 & 2.143 & 1.944 & 1.779 & 1.638 \\
 k_{101} & 1.363 & 0 & -1.513 & -2.96 & -4.324 & -5.618 & -6.857 & -8.056 & -9.221 & -10.362 \\
 k_{102} & 0.091 & 0 & -0.003 & 0.014 & -0.034 & 0.059 & -0.087 & 0.115 & -0.144 & 0.172 \\
 k_{103} & 5.515 & \text{n/a} & 1.587 & \text{n/a} & 1.251 & \text{n/a} & 1.142 & \text{n/a} & 1.092 & \text{n/a} \\
 k_{104} & -1.363 & -4 & -4.012 & -2.96 & -1.535 & 0 & 1.543 & 3.056 & 4.525 & 5.948 \\
 k_{105} & 0.091 & \text{n/a} & 0.333 & \text{n/a} & 0.472 & \text{n/a} & 0.564 & \text{n/a} & 0.628 & \text{n/a} \\
 k_{106} & \text{n/a} & 18 & \text{n/a} & 20.16 & \text{n/a} & 21.028 & \text{n/a} & 21.444 & \text{n/a} & 21.674 \\
 k_{107} & \text{n/a} & 0.426 & \text{n/a} & \text{n/a} & \text{n/a} & 0.618 & \text{n/a} & \text{n/a} & \text{n/a} & 0.704 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.338 & \text{n/a} & \text{n/a} & \text{n/a} & 1.86 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=2$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
\hline
 \text{J} & 0.496 & 0.447 & 0.386 & 0.333 & 0.292 & 0.259 & 0.232 & 0.21 & 0.192 & 0.177 \\
 \text{L} & 8.531 & 8.944 & 9.189 & 9.333 & 9.424 & 9.485 & 9.526 & 9.557 & 9.579 & 9.597 \\
 \text{JL} & 4.228 & 4 & 3.542 & 3.111 & 2.75 & 2.454 & 2.21 & 2.008 & 1.838 & 1.694 \\
 k_{101} & 1.228 & 0 & -1.458 & -2.889 & -4.25 & -5.546 & -6.79 & -7.992 & -9.162 & -10.306 \\
 k_{102} & 0.057 & 0 & -0.002 & 0.012 & -0.03 & 0.053 & -0.079 & 0.106 & -0.134 & 0.161 \\
 k_{103} & 8.757 & \text{n/a} & 1.702 & \text{n/a} & 1.287 & \text{n/a} & 1.161 & \text{n/a} & 1.103 & \text{n/a} \\
 k_{104} & -1.228 & -4 & -3.954 & -2.889 & -1.495 & 0 & 1.508 & 2.994 & 4.443 & 5.853 \\
 k_{105} & 0.057 & \text{n/a} & 0.309 & \text{n/a} & 0.455 & \text{n/a} & 0.549 & \text{n/a} & 0.616 & \text{n/a} \\
 k_{106} & \text{n/a} & 32 & \text{n/a} & 35.556 & \text{n/a} & 37.183 & \text{n/a} & 37.986 & \text{n/a} & 38.434 \\
 k_{107} & \text{n/a} & 0.32 & \text{n/a} & \text{n/a} & \text{n/a} & 0.612 & \text{n/a} & \text{n/a} & \text{n/a} & 0.697 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.732 & \text{n/a} & \text{n/a} & \text{n/a} & 1.927 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=3$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.333 & 0.316 & 0.283 & 0.25 & 0.221 & 0.198 & 0.178 & 0.162 & 0.148 & 0.137 \\
 \text{L} & 12.343 & 12.649 & 12.863 & 13 & 13.09 & 13.151 & 13.194 & 13.225 & 13.249 & 13.267 \\
 \text{JL} & 4.108 & 4. & 3.643 & 3.25 & 2.899 & 2.602 & 2.352 & 2.143 & 1.965 & 1.814 \\
 k_{101} & 1.108 & 0 & -1.357 & -2.75 & -4.101 & -5.398 & -6.648 & -7.857 & -9.035 & -10.186 \\
 k_{102} & 0.027 & 0 & -0.001 & 0.009 & -0.023 & 0.042 & -0.065 & 0.089 & -0.114 & 0.139 \\
 k_{103} & 18.604 & \text{n/a} & 1.977 & \text{n/a} & 1.372 & \text{n/a} & 1.203 & \text{n/a} & 1.129 & \text{n/a} \\
 k_{104} & -1.108 & -4 & -3.84 & -2.75 & -1.417 & 0 & 1.438 & 2.868 & 4.277 & 5.658 \\
 k_{105} & 0.027 & \text{n/a} & 0.263 & \text{n/a} & 0.419 & \text{n/a} & 0.519 & \text{n/a} & 0.59 & \text{n/a} \\
 k_{106} & \text{n/a} & 72 & \text{n/a} & 78.75 & \text{n/a} & 82.714 & \text{n/a} & 84.799 & \text{n/a} & 85.989 \\
 k_{107} & \text{n/a} & 0.18 & \text{n/a} & \text{n/a} & \text{n/a} & 0.595 & \text{n/a} & \text{n/a} & \text{n/a} & 0.684 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 4.874 & \text{n/a} & \text{n/a} & \text{n/a} & 2.082 & \text{n/a} & \text{n/a} \\
\end{array}
$$
